Cache-Aided Communications in MISO Networks with Dynamic User Behavior: A Universal Solution

A practical barrier to the implementation of cache-aided networks is dynamic and unpredictable user behavior. In dynamic setups, users can freely depart and enter the network at any moment. The shared caching concept has the potential to handle this issue by assigning $K$ users to $P$ caching profiles, where all $\eta_{p}$ users assigned to profile $p$ store the same cache content defined by that profile. The existing schemes, however, cannot be applied in general and are not dynamic in the true sense as they put constraints on the transmitter-side spatial multiplexing gain $\alpha$. Specifically, they work only if $\alpha \leq \min_{p} \eta_{p}$ or $\alpha \geq \hat{\eta}$, where in the latter case, $\gamma$ is the normalized cache size of each user, $\hat{\eta}$ is an arbitrary parameter satisfying $1 \leq \hat{\eta} \leq \max_{p} \eta_{p}$, and the extra condition of $\alpha \geq K\gamma$ should also be met. In this work, we propose a universal caching scheme based on the same shared-cache model that can be applied to any dynamic setup, extending the working region of existing schemes to networks with $\min_{p} \eta_{p} \leq \alpha \leq \hat{\eta}$ and removing any other constraints of existing schemes. We also derive the closed-form expressions for the achievable degrees-of-freedom (DoF) of the proposed scheme and show that it achieves the optimal DoF for uniform user distributions. Notably, it is the first scheme to achieve the optimal DoF of $K\gamma+\alpha$ for networks with uniform user distribution, $\alpha > \hat{\eta}$, and non-integer $\frac{\alpha}{\hat{\eta}}$, without imposing any other constraints. Finally, we use numerical simulations to assess how non-uniform user distribution impacts the DoF performance and illustrate that the proposed scheme provides a noticeable improvement over unicasting for uneven distributions.

==> MyCommands_old.tex <==
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}%[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}%[section]
\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem{rem}{Remark}

% Calligraphic Letters
\newcommand{\CA}[0]{{\mathcal{A}}}
\newcommand{\CB}[0]{{\mathcal{B}}}
\newcommand{\CC}[0]{{\mathcal{C}}}
\newcommand{\CD}[0]{{\mathcal{D}}}
\newcommand{\CE}[0]{{\mathcal{E}}}
\newcommand{\CF}[0]{{\mathcal{F}}}
\newcommand{\CG}[0]{{\mathcal{G}}}
\newcommand{\CH}[0]{{\mathcal{H}}}
\newcommand{\CI}[0]{{\mathcal{I}}}
\newcommand{\CJ}[0]{{\mathcal{J}}}
\newcommand{\CK}[0]{{\mathcal{K}}}
\newcommand{\CL}[0]{{\mathcal{L}}}
\newcommand{\CM}[0]{{\mathcal{M}}}
\newcommand{\CN}[0]{{\mathcal{N}}}
\newcommand{\CO}[0]{{\mathcal{O}}}
\newcommand{\CP}[0]{{\mathcal{P}}}
\newcommand{\CQ}[0]{{\mathcal{Q}}}
\newcommand{\CR}[0]{{\mathcal{R}}}
\newcommand{\CS}[0]{{\mathcal{S}}}
\newcommand{\CT}[0]{{\mathcal{T}}}
\newcommand{\CU}[0]{{\mathcal{U}}}
\newcommand{\CV}[0]{{\mathcal{V}}}
\newcommand{\CW}[0]{{\mathcal{W}}}
\newcommand{\CX}[0]{{\mathcal{X}}}
\newcommand{\CY}[0]{{\mathcal{Y}}}
\newcommand{\CZ}[0]{{\mathcal{Z}}}

% Boldface Letters
\newcommand{\Ba}[0]{{\mathbf{a}}}
\newcommand{\Bb}[0]{{\mathbf{b}}}
\newcommand{\Bc}[0]{{\mathbf{c}}}
\newcommand{\Bd}[0]{{\mathbf{d}}}
\newcommand{\Be}[0]{{\mathbf{e}}}
\newcommand{\Bf}[0]{{\mathbf{f}}}
\newcommand{\Bg}[0]{{\mathbf{g}}}
\newcommand{\Bh}[0]{{\mathbf{h}}}
\newcommand{\Bi}[0]{{\mathbf{i}}}
\newcommand{\Bj}[0]{{\mathbf{j}}}
\newcommand{\Bk}[0]{{\mathbf{k}}}
\newcommand{\Bl}[0]{{\mathbf{l}}}
\newcommand{\Bm}[0]{{\mathbf{m}}}
\newcommand{\Bn}[0]{{\mathbf{n}}}
\newcommand{\Bo}[0]{{\mathbf{o}}}
\newcommand{\Bp}[0]{{\mathbf{p}}}
\newcommand{\Bq}[0]{{\mathbf{q}}}
\newcommand{\Br}[0]{{\mathbf{r}}}
\newcommand{\Bs}[0]{{\mathbf{s}}}
\newcommand{\Bt}[0]{{\mathbf{t}}}
\newcommand{\Bu}[0]{{\mathbf{u}}}
\newcommand{\Bv}[0]{{\mathbf{v}}}
\newcommand{\Bw}[0]{{\mathbf{w}}}
\newcommand{\Bx}[0]{{\mathbf{x}}}
\newcommand{\By}[0]{{\mathbf{y}}}
\newcommand{\Bz}[0]{{\mathbf{z}}}

\newcommand{\BA}[0]{{\mathbf{A}}}
\newcommand{\BB}[0]{{\mathbf{B}}}
\newcommand{\BC}[0]{{\mathbf{C}}}
\newcommand{\BD}[0]{{\mathbf{D}}}
\newcommand{\BE}[0]{{\mathbf{E}}}
\newcommand{\BF}[0]{{\mathbf{F}}}
\newcommand{\BG}[0]{{\mathbf{G}}}
\newcommand{\BH}[0]{{\mathbf{H}}}
\newcommand{\BI}[0]{{\mathbf{I}}}
\newcommand{\BJ}[0]{{\mathbf{J}}}
\newcommand{\BK}[0]{{\mathbf{K}}}
\newcommand{\BL}[0]{{\mathbf{L}}}
\newcommand{\BM}[0]{{\mathbf{M}}}
\newcommand{\BN}[0]{{\mathbf{N}}}
\newcommand{\BO}[0]{{\mathbf{O}}}
\newcommand{\BP}[0]{{\mathbf{P}}}
\newcommand{\BQ}[0]{{\mathbf{Q}}}
\newcommand{\BR}[0]{{\mathbf{R}}}
\newcommand{\BS}[0]{{\mathbf{S}}}
\newcommand{\BT}[0]{{\mathbf{T}}}
\newcommand{\BU}[0]{{\mathbf{U}}}
\newcommand{\BV}[0]{{\mathbf{V}}}
\newcommand{\BW}[0]{{\mathbf{W}}}
\newcommand{\BX}[0]{{\mathbf{X}}}
\newcommand{\BY}[0]{{\mathbf{Y}}}
\newcommand{\BZ}[0]{{\mathbf{Z}}}

% Bar over the letters
\newcommand{\Bra}[0]{{\Bar{a}}}
\newcommand{\Brb}[0]{{\Bar{b}}}
\newcommand{\Brc}[0]{{\Bar{c}}}
\newcommand{\Brd}[0]{{\Bar{d}}}
\newcommand{\Bre}[0]{{\Bar{e}}}
\newcommand{\Brf}[0]{{\Bar{f}}}
\newcommand{\Brg}[0]{{\Bar{g}}}
\newcommand{\Brh}[0]{{\Bar{h}}}
\newcommand{\Bri}[0]{{\Bar{i}}}
\newcommand{\Brj}[0]{{\Bar{j}}}
\newcommand{\Brk}[0]{{\Bar{k}}}
\newcommand{\Brl}[0]{{\Bar{l}}}
\newcommand{\Brm}[0]{{\Bar{m}}}
\newcommand{\Brn}[0]{{\Bar{n}}}
\newcommand{\Bro}[0]{{\Bar{o}}}
\newcommand{\Brp}[0]{{\Bar{p}}}
\newcommand{\Brq}[0]{{\Bar{q}}}
\newcommand{\Brr}[0]{{\Bar{r}}}
\newcommand{\Brs}[0]{{\Bar{s}}}
\newcommand{\Brt}[0]{{\Bar{t}}}
\newcommand{\Bru}[0]{{\Bar{u}}}
\newcommand{\Brv}[0]{{\Bar{v}}}
\newcommand{\Brw}[0]{{\Bar{w}}}
\newcommand{\Brx}[0]{{\Bar{x}}}
\newcommand{\Bry}[0]{{\Bar{y}}}
\newcommand{\Brz}[0]{{\Bar{z}}}

\newcommand{\BrA}[0]{{\Bar{A}}}
\newcommand{\BrB}[0]{{\Bar{B}}}
\newcommand{\BrC}[0]{{\Bar{C}}}
\newcommand{\BrD}[0]{{\Bar{D}}}
\newcommand{\BrE}[0]{{\Bar{E}}}
\newcommand{\BrF}[0]{{\Bar{F}}}
\newcommand{\BrG}[0]{{\Bar{G}}}
\newcommand{\BrH}[0]{{\Bar{H}}}
\newcommand{\BrI}[0]{{\Bar{I}}}
\newcommand{\BrJ}[0]{{\Bar{J}}}
\newcommand{\BrK}[0]{{\Bar{K}}}
\newcommand{\BrL}[0]{{\Bar{L}}}
\newcommand{\BrM}[0]{{\Bar{M}}}
\newcommand{\BrN}[0]{{\Bar{N}}}
\newcommand{\BrO}[0]{{\Bar{O}}}
\newcommand{\BrP}[0]{{\Bar{P}}}
\newcommand{\BrQ}[0]{{\Bar{Q}}}
\newcommand{\BrR}[0]{{\Bar{R}}}
\newcommand{\BrS}[0]{{\Bar{S}}}
\newcommand{\BrT}[0]{{\Bar{T}}}
\newcommand{\BrU}[0]{{\Bar{U}}}
\newcommand{\BrV}[0]{{\Bar{V}}}
\newcommand{\BrW}[0]{{\Bar{W}}}
\newcommand{\BrX}[0]{{\Bar{X}}}
\newcommand{\BrY}[0]{{\Bar{Y}}}
\newcommand{\BrZ}[0]{{\Bar{Z}}}

% Serif Letters
\newcommand{\Sfa}[0]{{\mathsf{a}}}
\newcommand{\Sfb}[0]{{\mathsf{b}}}
\newcommand{\Sfc}[0]{{\mathsf{c}}}
\newcommand{\Sfd}[0]{{\mathsf{d}}}
\newcommand{\Sfe}[0]{{\mathsf{e}}}
\newcommand{\Sff}[0]{{\mathsf{f}}}
\newcommand{\Sfg}[0]{{\mathsf{g}}}
\newcommand{\Sfh}[0]{{\mathsf{h}}}
\newcommand{\Sfi}[0]{{\mathsf{i}}}
\newcommand{\Sfj}[0]{{\mathsf{j}}}
\newcommand{\Sfk}[0]{{\mathsf{k}}}
\newcommand{\Sfl}[0]{{\mathsf{l}}}
\newcommand{\Sfm}[0]{{\mathsf{m}}}
\newcommand{\Sfn}[0]{{\mathsf{n}}}
\newcommand{\Sfo}[0]{{\mathsf{o}}}
\newcommand{\Sfp}[0]{{\mathsf{p}}}
\newcommand{\Sfq}[0]{{\mathsf{q}}}
\newcommand{\Sfr}[0]{{\mathsf{r}}}
\newcommand{\Sfs}[0]{{\mathsf{s}}}
\newcommand{\Sft}[0]{{\mathsf{t}}}
\newcommand{\Sfu}[0]{{\mathsf{u}}}
\newcommand{\Sfv}[0]{{\mathsf{v}}}
\newcommand{\Sfw}[0]{{\mathsf{w}}}
\newcommand{\Sfx}[0]{{\mathsf{x}}}
\newcommand{\Sfy}[0]{{\mathsf{y}}}
\newcommand{\Sfz}[0]{{\mathsf{z}}}

\newcommand{\SfA}[0]{{\mathsf{A}}}
\newcommand{\SfB}[0]{{\mathsf{B}}}
\newcommand{\SfC}[0]{{\mathsf{C}}}
\newcommand{\SfD}[0]{{\mathsf{D}}}
\newcommand{\SfE}[0]{{\mathsf{E}}}
\newcommand{\SfF}[0]{{\mathsf{F}}}
\newcommand{\SfG}[0]{{\mathsf{G}}}
\newcommand{\SfH}[0]{{\mathsf{H}}}
\newcommand{\SfI}[0]{{\mathsf{I}}}
\newcommand{\SfJ}[0]{{\mathsf{J}}}
\newcommand{\SfK}[0]{{\mathsf{K}}}
\newcommand{\SfL}[0]{{\mathsf{L}}}
\newcommand{\SfM}[0]{{\mathsf{M}}}
\newcommand{\SfN}[0]{{\mathsf{N}}}
\newcommand{\SfO}[0]{{\mathsf{O}}}
\newcommand{\SfP}[0]{{\mathsf{P}}}
\newcommand{\SfQ}[0]{{\mathsf{Q}}}
\newcommand{\SfR}[0]{{\mathsf{R}}}
\newcommand{\SfS}[0]{{\mathsf{S}}}
\newcommand{\SfT}[0]{{\mathsf{T}}}
\newcommand{\SfU}[0]{{\mathsf{U}}}
\newcommand{\SfV}[0]{{\mathsf{V}}}
\newcommand{\SfW}[0]{{\mathsf{W}}}
\newcommand{\SfX}[0]{{\mathsf{X}}}
\newcommand{\SfY}[0]{{\mathsf{Y}}}
\newcommand{\SfZ}[0]{{\mathsf{Z}}}

%=====================================================================================================================================
% ===========================================================================
% File Name: commands.tex
% File Creation Date: 15.6.1995
% Author: Markku Juntti
% Description: Includes useful commands for Latex edition.
% ===========================================================================

\renewcommand{\Re}{\mbox{Re}}
\renewcommand{\Im}{\mbox{Im}}

% Bold-face Greek letters
\renewcommand{\vec}[1]{\bf{#1}}     %equation styles %vector/matrix

% Figure-specific commands
%\newcommand{\MyRect}[2]{}
\newcommand{\FillGray}[3]{\filldraw[gray!50](#3-1+0.1,#1-#2+0.1) rectangle (#3-0.1,#1-#2+1-0.1)}
\newcommand{\FillBlack}[3]{\filldraw[black!70](#3-1+0.1,#1-#2+0.1) rectangle (#3-0.1,#1-#2+1-0.1)}
\newcommand{\FillHatch}[3]{\fill[pattern=crosshatch, pattern color=black!65](#3-1,#1-#2)rectangle(#3,#1-#2+1)}
\ExplSyntaxOn

\NewDocumentCommand \vect { s o m }
 {
  \IfBooleanTF {#1}
   { \vectaux*{#3} }
   { \IfValueTF {#2} { \vectaux[#2]{#3} } { \vectaux{#3} } }
 }
\DeclarePairedDelimiterX \vectaux [1] {\lbrack} {\rbrack}
 { \, \dbacc_vect:n { #1 } \, }
\cs_new_protected:Npn \dbacc_vect:n #1
 {
  \seq_set_split:Nnn \l_tmpa_seq { , } { #1 }
  \seq_use:Nn \l_tmpa_seq { \enspace }
 }
\ExplSyntaxOff


==> abbrev.tex <==
%!TeX root = d2d-cc.tex

% Declaration of the abbreviations
\DeclareAcronym{AWGN}{
    short = AWGN,
    long = additive white Gaussian noise,
    list = Additive White Gaussian Noise,
  %  tag = abbrev
}

\DeclareAcronym{ADMM}{
    short = ADMM,
    long = alternating direction method of multipliers,
    list = Alternating Direction Method of Multipliers,
   % tag = abbrev
}

\DeclareAcronym{MGMC}{
    short = MGMC,
    long = multi-group multi-casting,
    list = multi-group multi-casting,
    %tag = abbrev
}

\DeclareAcronym{SGMC}{
    short = SGMC,
    long = single-group multi-casting,
    list = single-group multi-casting,
    %tag = abbrev
}
\DeclareAcronym{AoA}{
    short = AoA,
    long = angle-of-arrival,
    list = Angle-of-Arrival,
    %tag = abbrev
}

\DeclareAcronym{AoD}{
    short = AoD,
    long = angle-of-departure,
    list = Angle-of-Departure,
    %tag = abbrev
}

\DeclareAcronym{KKT}{
    short = KKT,
    long = Karush-Kuhn-Tucker,
    list = Karush-Kuhn-Tucker,
    %tag = abbrev
}

\DeclareAcronym{MMF}{
    short = MMF,
    long = max-min-fairness,
    list = max-min-fairness,
   % tag = abbrev
}

\DeclareAcronym{WMMF}{
    short = WMMF,
    long = weighted max-min-fairness,
    list = max-min-fairness,
    %tag = abbrev
}

\DeclareAcronym{BB}{
    short = BB,
    long = base band,
    list = Base Band,
    %tag = abbrev
}

\DeclareAcronym{BC}{
    short = BC,
    long = broadcast channel,
    list = Broadcast Channel,
   % tag = abbrev
}

\DeclareAcronym{BS}{
    short = BS,
    long = base station,
    list = Base Station,
    %tag = abbrev
}

\DeclareAcronym{BR}{
    short = BR,
    long = best response,
    list = Best Response, 
    %tag = abbrev
}

\DeclareAcronym{CB}{
    short = CB,
    long = coordinated beamforming,
    list = Coordinated Beamforming,
   % tag = abbrev
}

\DeclareAcronym{CC}{
    short = CC,
    long = coded caching,
    list = Coded Caching,
    %tag = abbrev
}

\DeclareAcronym{CE}{
    short = CE,
    long = channel estimation,
    list = Channel Estimation,
   % tag = abbrev
}

\DeclareAcronym{CoMP}{
    short = CoMP,
    long = coordinated multi-point transmission,
    list = Coordinated Multi-Point Transmission,
    %tag = abbrev
}

\DeclareAcronym{CRAN}{
    short = C-RAN,
    long = cloud radio access network,
    list = Cloud Radio Access Network,
    %tag = abbrev
}

\DeclareAcronym{CSE}{
    short = CSE,
    long = channel specific estimation,
    list = Channel Specific Estimation,
    %tag = abbrev
}

\DeclareAcronym{CSI}{
    short = CSI,
    long = channel state information,
    list = Channel State Information,
   % tag = abbrev
}

\DeclareAcronym{CSIT}{
    short = CSIT,
    long = channel state information at the transmitter,
    list = Channel State Information at the Transmitter,
   % tag = abbrev
}

\DeclareAcronym{CU}{
    short = CU,
    long = central unit,
    list = Central Unit,
   %tag = abbrev
}

\DeclareAcronym{D2D}{
    short = D2D,
    long = device-to-device,
    list = Device-to-Device,
   % tag = abbrev
}

\DeclareAcronym{DE-ADMM}{
    short = DE-ADMM,
    long = direct estimation with alternating direction method of multipliers,
    list = Direct Estimation with Alternating Direction Method of Multipliers,
   % tag = abbrev
}

\DeclareAcronym{DE-BR}{
    short = DE-BR,
    long = direct estimation with best response,
    list = Direct Estimation with Best Response,
   % tag = abbrev
}

\DeclareAcronym{DE-SG}{
    short = DE-SG,
    long = direct estimation with stochastic gradient,
    list = Direct Estimation with Stochastic Gradient,
   % tag = abbrev
}

\DeclareAcronym{DFT}{
	short = DFT,
	long = discrete fourier transform,
	list = Discrete Fourier Transform,
	%tag = abbrev
}

\DeclareAcronym{DoF}{
    short = DoF,
    long = degrees of freedom,
    list = Degrees of Freedom,
   % tag = abbrev
}

\DeclareAcronym{DL}{
    short = DL,
    long = downlink,
    list = Downlink,
    %tag = abbrev
}

\DeclareAcronym{GD}{
	short = GD, 
	long = gradient descent,
	list = Gradeitn Descent,
	%tag = abbrev
}

\DeclareAcronym{IBC}{
    short = IBC,
    long = interfering broadcast channel,
    list = Interfering Broadcast Channel,
    %tag = abbrev
}

\DeclareAcronym{i.i.d.}{
    short = i.i.d.,
    long = independent and identically distributed,
    list = Independent and Identically Distributed,
   %tag = abbrev
}

\DeclareAcronym{JP}{
    short = JP,
    long = joint processing,
    list = Joint Processing,
 %   tag = abbrev
}


\DeclareAcronym{LOS}{
	short = LOS,
	long = line-of-sight,
	list = Line-of-Sight,
%	tag = abbrev
}

\DeclareAcronym{LS}{
    short = LS,
    long = least squares,
    list = Least Squares,
   % tag = abbrev
}

\DeclareAcronym{LTE}{
    short = LTE,
    long = Long Term Evolution,
   % tag = abbrev
}

\DeclareAcronym{LTE-A}{
    short = LTE-A,
    long = Long Term Evolution Advanced,
  %  tag = abbrev
}

\DeclareAcronym{MIMO}{
    short = MIMO,
    long = multiple-input multiple-output,
    list = Multiple-Input Multiple-Output,
  %  tag = abbrev
}

\DeclareAcronym{MISO}{
    short = MISO,
    long = multiple-input single-output,
    list = Multiple-Input Single-Output,
  %  tag = abbrev
}

\DeclareAcronym{MAC}{
    short = MAC,
    long = multiple access channel,
    list = Multiple Access Channel,
  %  tag = abbrev
}

\DeclareAcronym{MSE}{
    short = MSE,
    long = mean-squared error,
    list = Mean-Squared Error,
   % tag = abbrev
}

\DeclareAcronym{MMSE}{
    short = MMSE,
    long = minimum mean-squared error,
    list = Minimum Mean-Squared Error,
   % tag = abbrev
}

\DeclareAcronym{mmWave}{
	short = mmWave,
	long = millimeter wave,
	list = Millimeter Wave,
	%tag = abbrev
}

\DeclareAcronym{MU-MIMO}{
    short = MU-MIMO,
    long = multi-user \ac{MIMO},
    list = Multi-User \ac{MIMO},
   % tag = abbrev
}

\DeclareAcronym{OTA}{
    short = OTA,
    long = over-the-air,
    list = Over-the-Air,
   % tag = abbrev
}

\DeclareAcronym{PSD}{
    short = PSD,
    long = positive semidefinite,
    list = Positive Semidefinite,
   % tag = abbrev
}

\DeclareAcronym{QoS}{
	short = QoS,
	long = quality of service,
	list = Quality of Service,
	%tag = abbrev
}

\DeclareAcronym{RCP}{
	short = RCP,
	long = remote central processor,
	list = Remote Central Processor,
	%tag = abbrev
}

\DeclareAcronym{RRH}{
    short = RRH,
    long = remote radio head,
    list = Remote Radio Head,
   % tag = abbrev
}

\DeclareAcronym{RSSI}{
    short = RSSI,
    long = received signal strength indicator,
    list = Received Signal Strength Indicator,
   % tag = abbrev
}

\DeclareAcronym{RX}{
	short = RX,
	long = receiver,
	list = Receiver,
	%tag = abbrev
}

\DeclareAcronym{SCA}{
    short = SCA,
    long = successive-convex-approximation,
    list = Successive-Convex-Approximation,
  %  tag = abbrev
}

\DeclareAcronym{SG}{
    short = SG,
    long = stochastic gradient,
    list = Stochastic Gradient,
    %tag = abbrev
}

\DeclareAcronym{SIC}{
    short = SIC,
    long = successive interference cancellation,
    list = Successive Interference Cancellation,
  %  tag = abbrev
}

\DeclareAcronym{SNR}{
    short = SNR,
    long = signal-to-noise-ratio,
    list = Signal-to-Noise Ratio,
   % tag = abbrev
}

\DeclareAcronym{SDR}{
    short = SDR,
    long = semi-definite-relaxation,
    list = semi-definite-relaxation,
   % tag = abbrev
}

\DeclareAcronym{SINR}{
    short = SINR,
    long = signal-to-interference-plus-noise ratio,
    list = Signal-to-Interference-plus-Noise Ratio,
 %   tag = abbrev
}

\DeclareAcronym{SOCP}{
	short = SOCP, 
	long = second order cone program,
	list = Second Order Cone Program,
	%tag = abbrev
}

\DeclareAcronym{SSE}{
    short = SSE,
    long = stream specific estimation,
    list = Stream Specific Estimation,
   % tag = abbrev
}

\DeclareAcronym{SVD}{
	short = SVD,
	long = singular value decomposition,
	list = Singular Value Decomposition,
	%tag = abbrev
}

\DeclareAcronym{TDD}{
	short = TDD,
	long = time division duplex,
	list = Time Division Duplex,
%	tag = abbrev
}

\DeclareAcronym{TX}{
	short = TX,
	long = transmitter,
	list = Transmitter,
	%tag = abbrev
}

\DeclareAcronym{UE}{
    short = UE,
    long = user equipment,
    list = User Equipment,
  %  tag = abbrev
}

\DeclareAcronym{UL}{
    short = UL,
    long = uplink,
    list = Uplink,
  %  tag = abbrev
}

\DeclareAcronym{ULA}{
	short = ULA,
	long = uniform linear array,
	list = Uniform Linear Array,
%	tag = abbrev
}

\DeclareAcronym{UPA}{
    short = UPA,
    long = uniform planar array,
    list = Uniform Planar Array,
  %  tag = abbrev
}

\DeclareAcronym{WMMSE}{
    short = WMMSE,
    long = weighted minimum mean-squared error,
    list = Weighted Minimum Mean-Squared Error,
  %  tag = abbrev
}

\DeclareAcronym{WMSEMin}{
    short = WMSEMin,
    long = weighted sum \ac{MSE} minimization,
    list = Weighted sum \ac{MSE} Minimization,
  %  tag = abbrev
}

\DeclareAcronym{WBAN}{
	short = WBAN,
	long = wireless body area network,
	list = Wireless Body Area Network,
	%tag = abbrev
}

\DeclareAcronym{WSRMax}{
    short = WSRMax,
    long = weighted sum rate maximization,
    list = Weighted Sum Rate Maximization,
  %  tag = abbrev
}
